New second-order optimality conditions in sub-Riemannian Geometry

We study the geometry of the second-order expansion of the extended end-point map for the sub-Riemannian geodesic problem. Translating the geometric reality into equations we derive new second-order necessary optimality conditions in sub-Riemannian Geometry. In particular, we find an ODE for velocity of an abnormal sub-Riemannian geodesics. It allows to divide abnormal minimizers into two classes, which we propose to call 2-normal and 2-abnormal extremals. In the 2-normal case the above ODE completely determines the velocity of a curve, while in the 2-abnormal case the velocity is undetermined at some, or at all points. With some enhancement of the presented results it should be possible to prove the regularity of all 2-normal extremals (the 2-abnormal case seems to require study of higher-order conditions) thus making a step towards solving the problem of smoothness of sub-Riemannian abnormal geodesics. As a by-product we present a new derivation of Goh conditions. We also prove that the assumptions weaker than these used in [Boarotto, Monti, Palmurella, 2020] to derive third-order Goh conditions, imply piece-wise-$C^2$ regularity of an abnormal extremal.

==> second_order_case.tex <==
\section{The main result}\label{sec:results}

Vanishing of the Agrachew-Sarychew index and the finiteness of all the minimal 2-jets, provides a lot of information about an abnormal extremal. In particular, we get Goh conditions, and also a condition for regularity of the trajectory analogous to the normal-abnormal alternative in the first order case.

\begin{theorem}\label{thm:optimal_deg_2} Let $q(t)$ corresponding to the control $u(t)\in\LL{t_0}{t_1}$ be a strictly abnormal SR extremal. Assume further that $\phi(t)$ is a related adjoint curve such that the Agrachew-Sarychew index $\I(t_0,t_1)=0$, and that the minimal 2-jet $\bmin(t,\wt b_1)$ exists for every $t\in [t_0,t_1)$ and every $\wt b_1\in\BF(t_0,t)=\operatorname{Im}\dd_0\End{t_0,t}{\wt q_0}$.
\smallskip

Then there exist continuous, almost everywhere differentiable curves: a curve of covectors $\xi(t)\in \T^\ast_{q(t)}M$, a curve of symmetric bi-linear maps $\Phi(t):\T_{q(t)}M\times\T_{q(t)} M\ra \R$, and a real curve $a_2(t)\in\R$ such that for each $i=1,2,\hdots,k$
\begin{align}
%\label{eqn:phi_abnormal} \<X_i,\phi(t)>=&0\\
\label{eqn:xi_u_1}
\<X_i\big|_{q(t)},\xi(t)>+2\ a_2(t)\cdot u_i(t)=&0\\
\label{eqn:Phi_b_1}
2\<\frac{\pa X_i}{\pa q}\Big|_{q(t)}b_1,\phi(t)>+2\Phi(t)\left[X_i\big|_{q(t)},b_1\right]+\<b_1,\xi(t)>\ u_i(t)=&0\quad \text{for every $b_1\in B_1(t_0,t)$}
\end{align} 
Moreover, at the points $t\in[t_0,t_1]$ of differentiability of the above-mentioned curves, the symmetric bi-linear form  
\begin{equation}
\label{eqn:2_form_positive}
\<\sum_{i=1}^k u_i(t) \frac{\pa^2 X_i}{\pa q^2} b_1b_1,\phi>-\dot\Phi[b_1,b_1]-2\Phi\left[\sum_{i=1}^k u_i(t)\frac{\pa X_i}{\pa q}b_1,b_1\right]-\left(\<b_1,\dot\xi>+\<\sum_{i=1}^k u_i(t)\frac{\pa X_i}{\pa q}b_1,\xi>\right)\cdot c_1-\dot{a_2}\cdot c_1^2
\end{equation}
is non-negatively defined on $\BF(t_0,t)\ni \wt b_1=b_1+c_1\cdot\pa_r$. 
\end{theorem}

\begin{remark}\label{rem:deg2_full}
\begin{enumerate}[(i)]
	\item If $a_2(t)\neq 0$ then \eqref{eqn:xi_u_1}  implies that $u_i(t)$ is continuous and a.e. differentiable, hence $q(t)$ is $C^1$, with $\ddot q(t)$ defined almost everywhere. 
	\item Regardless of the value of $a_2(t)$,  equations \eqref{eqn:xi_u_1}-\eqref{eqn:Phi_b_1} imply \emph{Goh conditions}. Indeed, put $b_1=X_j$ {\new komentarz} in \eqref{eqn:Phi_b_1} to get
\begin{align*}
2\<\frac{\pa X_i}{\pa q}X_j,\phi>\overset{\eqref{eqn:Phi_b_1}}=-2\Phi\left[ X_i,X_j\right]-\<X_j,\xi>u_i(t)\overset{\eqref{eqn:xi_u_1}}=-2\Phi\left[ X_i,X_j\right]+a_2\cdot u_j(t)u_i(t)\ .
\end{align*}	
The right-hand side of the above expression is symmetric, hence 
 $$\<[X_i,X_j],\phi>=\<\frac{\pa X_i}{\pa q}X_j,\phi>-\<\frac{\pa X_j}{\pa q}X_i,\phi>=0\ .$$
	\item\label{point:iii} If $a_2(t)\equiv0$ (or more generally if $\dot a_2(t)=0$), then the bi-linear form \eqref{eqn:2_form_positive} contains a bare term linear in $c_1$. This term should vanish for every possible choice of $b_1$, since otherwise the form would not be positively defined. This reasoning gives the evolution equation for $\xi(t)$:
	\begin{equation}
	\label{eqn:ev_xi_1}
\<b_1,\dot\xi(t)>+\<\sum_{i=1}^ku_i(t)\cdot \frac{\pa X_i}{\pa q}b_1,\xi(t)>=0 
	\end{equation}
	for every $b_1\in B_1(t_0,t)$. 
\smallskip

Thus in case $a_2(t)\equiv 0$, equations~\eqref{eqn:ev_xi_1} and \eqref{eqn:xi_u_1} are the same as equations for an abnormal extremal form Thm.~\ref{thm:optimal_deg_1}. In such a situation we shall say that $q(t)$ is a \emph{2-abnormal extremal}, otherwise we speak about a \emph{2-normal extremal}. Let us remark that the name ``2-abnormal'' has also a control-theoretic justification -- see  {\new uwaga}.
\end{enumerate}
\end{remark}


\begin{proof}[Proof of Thm.~\ref{thm:optimal_deg_2}] By the results of Lem.~\ref{lem:2_jet_quadratic}, there exists a family of quadratic forms $\wt \Phi(t):\BF(t_0,t)\times\BF(t_0,t)\ra\R$ such that $\bmin(t,\wt b_1)=\wt \Phi(t)[\wt b_1,\wt b_1]$. We may decompose $\wt \Phi(t)$ according to Rem.~\ref{rem:2_covector_decomposition} getting
$$\wt \Phi(t)=\Phi(t)+\xi(t)\overset{\cdot}\otimes\dd r+a_2(t)\cdot\dd r\otimes\dd r\ .$$
The second part of Lem.~\ref{lem:2_jet_quadratic} guarantees that $\wt \Phi(t)$  (and thus also  the curves $\Phi(t)$, $\xi(t)$, and $a_2(t)$) is of bounded variation  and differentiable almost everywhere with respect to $t$. 
\medskip

Take now any control $\du\in \LL{t_0}{t_1}$. By the Fundamental Lem.~\ref{lem:fundamental} function 
\begin{align*}
t\longmapsto &\<\wt b_2(t,\du),\phi(t)>-\bmin(t,\wt b_1(t,\du))\overset{\text{Lem.}~\ref{lem:2_jet_quadratic}}=\<\wt b_2(t,\du),\phi(t)>-\wt \Phi(t)\left[\wt b_1(t,\du),\wt b_1(t,\du)\right]=\\
&\<\wt b_2(t,\du),\phi(t)>-\Phi(t)[b_1(t,\du),b_1(t,\du)]-\<b_1(t,\du),\xi(t)>c_1(t,\du)-a_2(t)\cdot c_1(t,\du)^2
\end{align*}
is non-decreasing. What is more, it is  differentiable a.e, hence its $t$-derivative has to be non-negative. This gives us
\begin{align*}
0\leq&\<b_2,\dot\phi>+\<\dot{b_2},\phi>-\dot\Phi[b_1,b_1]-2\Phi[\dot{b_1},b_1]-\<b_1,\dot\xi>c_1-\<\dot b_1,\xi>c_1-\<b_1,\xi>\dot{c_1}-\dot{a_2}\cdot c_1^2-2a_2\cdot c_1\dot{c_1}\overset{\eqref{eqn:b1},\eqref{eqn:b2}}=\\
&\underbrace{\<b_2,\dot\phi>+\<\sum_{i=1}^k u_i(t)\frac{\pa X_i}{\pa q}b_2,\phi>}_{\eqref{eqn:ev_phi}}+\<\sum_{i=1}^k u_i(t) \frac{\pa^2 X_i}{\pa q^2} b_1b_1+2\sum_{i=1}^k \du_i(t)\frac{\pa X_i}{\pa q}b_1,\phi>+\\
&-\dot\Phi[b_1,b_1]-2\Phi\left[\sum_{i=1}^k u_i(t)\frac{\pa X_i}{\pa q}b_1+\sum_{i=1}^k \du_i(t) X_i,b_1\right]+\\
&-\<b_1,\dot\xi>c_1-\<\sum_{i=1}^k u_i(t)\frac{\pa X_i}{\pa q}b_1,\xi>c_1-\<\sum_{i=1}^k \du_i(t)X_i,\xi>c_1-\<b_1,\xi>\sum_{i=1}^k \du_i(t)u_i(t)+\\
&-\dot{a_2}\cdot c_1^2-2 a_2\cdot c_1\sum_{i=1}^k \du_i(t)u_i(t)=\\
&\underbrace{\<\sum_{i=1}^k u_i(t) \frac{\pa^2 X_i}{\pa q^2} b_1b_1,\phi>-\dot\Phi[b_1,b_1]-2\Phi\left[\sum_{i=1}^k u_i(t)\frac{\pa X_i}{\pa q}b_1,b_1\right]-\left(\<b_1,\dot\xi>+\<\sum_{i=1}^k u_i(t)\frac{\pa X_i}{\pa q}b_1,\xi>\right)c_1-\dot{a_2}\cdot c_1^2}_{\text{quadratic in $b_1$ and $c_1$}}+\\
&-\underbrace{\sum_{i=1}^k \du_i(t)\left\{2\<\frac{\pa X_i}{\pa q}b_1,\phi>+\Phi\left[X_i,b_1\right]+\<b_1,\xi>u_i(t)+c_1\left(\<X_i,\xi>+2a_2\cdot u_i(t)\right)\right\}}_{\text{linear in $\du(t)$}}
\end{align*}
At a given $b_1+c_1\cdot\pa_r\in\BF(t_0,t)$, we may choose arbitrary $\du_i(t)$, hence the part linear in $\du_i(t)$ should vanish, leaving us with 
$$2\<\frac{\pa X_i}{\pa q}b_1,\phi>+\Phi\left[X_i,b_1\right]+\<b_1,\xi>u_i(t)+c_1\left(\<X_i,\xi>+2a_2\cdot u_i(t)\right)=0\qquad\text{for any $b_1+c_1\cdot\pa_r\in\BF(t_0,t)$}$$
Taking $b_1=0$ and $c_1\neq0$, and then $c_1=0$, $b_1\neq 0$ {\new komentarz}, leaves us with \eqref{eqn:xi_u_1} and \eqref{eqn:Phi_b_1} for almost every $t\in[t_0,t_1]$. 
\smallskip

Further, as the linear part of the above expression vanishes, the remaining quadratic part should be non-negatively defined, leading to \eqref{eqn:2_form_positive}. 
\medskip

{\new So far, we know only that $\wt \Phi(t)$ is a piece-wise continuous map. Now we would like to prove that actually it is of class $C^0$. Our argument will use a construction similar to a weak derrivative.} By the results of Lem.~\ref{lem:2_jet_quadratic} $\wt \Phi_{\alpha\beta}(t)$ is a function of bounded-variation. In particular, it has left and right limits at any point in its domain, and further it is discontinuous in at most countable number of points \cite{Lojasiewicz_1988}. 

Note that if $\wt \Phi(t)$ is differentialble then for every $\wt b_1(t)=\wt b_1(t,\du)$ (vanishing at the end-point) we have
$$\int_{t_0}^{t_1}\dot{\wt\Phi}(t)[\wt b_1(t),\wt b_1(t)]\ \dd t=-\int_{t_0}^{t_1}2\wt \Phi(t)[\dot {\wt b_1}(t),\wt b_1(t)]\dd t\ .$$ 
Let us calculate the right-hand side of the above expression
\begin{align*}
2\wt \Phi(t)&[\dot {\wt b_1}(t),\wt b_1(t)]=2\Phi(t)[\dot{b_1},b_1] + \<\dot b_1,\xi>c_1+\<b_1,\xi>\dot{c_1}+2 a_2\cdot c_1\dot{c_1}\overset{\eqref{eqn:b1}}=\\
&2\Phi(t)\left[\sum_{i=1}^ku_i\frac{\pa X_i}{\pa q}b_1+\sum_i \du_i X_i,b_1\right]+\<\sum_{i=1}^ku_i\frac{\pa X_i}{\pa q}b_1+\sum_i \du_i X_i,\xi>c_1+\\
&\qquad\<b_1,\xi>\sum_i u_i\du_i+2 a_2\cdot c_1 \sum_i u_i\du_i=\\
&\sum_i \du_i\Big\{ \underbrace{2\Phi(t)[X_i,b_1]+\<b_1,\xi >u_i}_{=-2\<\frac{\pa X_i}{\pa q}b_1,\phi>\text{ a.e by \eqref{eqn:Phi_b_1}}}+ c_1\big(\underbrace{\<X_i,\xi>+2a_2\cdot u_i}_{=0\text{ a.e by \eqref{eqn:xi_u_1}}}\big) \Big\}+\\
&\qquad 2\Phi(t)\left[\sum_i u_i\frac{\pa X_i}{\pa q}b_1,b_1\right]+\<\sum_i u_i\frac{\pa X_i}{\pa q}b_1,\xi>c_1=\\
&-2\sum_i\du_i\<\frac{\pa X_i}{\pa q}b_1,\phi>+ 2\Phi(t)\left[\sum_i u_i\frac{\pa X_i}{\pa q}b_1,b_1\right]+\<\sum_i u_i\frac{\pa X_i}{\pa q}b_1,\xi>c_1=\\
&\underbrace{-\<b_2,\dot\phi>-\<\sum_i u_i\frac{\pa X_i}{\pa q}b_2,\phi>}_{=0 \text{ by \eqref{eqn:ev_phi}}}-\<\sum_i u_i\frac{\pa^2 X_i}{\pa q^2}b_1b_1,\phi>+\<\sum_i u_i\frac{\pa^2 X_i}{\pa q^2}b_1b_1,\phi>+\\
&\qquad -2\sum_i\du_i\<\frac{\pa X_i}{\pa q}b_1,\phi>+ 2\Phi(t)\left[\sum_i u_i\frac{\pa X_i}{\pa q}b_1,b_1\right]+\<\sum_i u_i\frac{\pa X_i}{\pa q}b_1,\xi>c_1=\\
&-\<b_2,\dot\phi>-\<\dot{b_2},\phi>+\<\sum_i u_i\frac{\pa^2 X_i}{\pa q^2}b_1b_1,\phi>+ 2\Phi(t)\left[\sum_i u_i\frac{\pa X_i}{\pa q}b_1,b_1\right]+\<\sum_i u_i\frac{\pa X_i}{\pa q}b_1,\xi>c_1=\\
&-\frac{\dd}{\dd t}\<b_2,\phi>+\<\sum_i u_i\frac{\pa^2 X_i}{\pa q^2}b_1b_1,\phi>+ 2\Phi(t)\left[\sum_i u_i\frac{\pa X_i}{\pa q}b_1,b_1\right]+\<\sum_i u_i\frac{\pa X_i}{\pa q}b_1,\xi>c_1
\end{align*}


\end{proof}

Passing to arbitrary abnormal minimiznig SR geodesics is now easy after using the divisions provided by Lemmas~\ref{lem:AS_index_zero} and \ref{lem:existence_min_2_jets}.

\begin{theorem}\label{thm:abnormal_piecewise_smmoth} Let $q(t)$ be a locally strictly abnormal minimiznig SR geodesics corresponding to the control $u(t)\in\LL{t_0}{t_1}$. Then there exists a related adjoint curve $\phi(t)$, and a division of $[t_0,t_1]$ into a finite number of parts (at most $(n-k)(n-k+2)$) such that on each of them the assertion of Thm.~\ref{thm:optimal_deg_2} holds. In particular if $q(t)$ is not 2-abnormal, it is piecewise $C^1$. 
\end{theorem}
%{\new Z wynikiem \cite{no_corners_2016}, prawdopodobnie to daje globalnie $C^1$.} 
\begin{proof}
We use Lem.~\ref{lem:AS_index} to prove the existence of the adjoint curve $\phi(t)$ for which $\I(t_0,t_1)$ is finite. Then we divide $[t_0,t_1]$ as in Lemma~\ref{lem:AS_index_zero} to put the Agrachew-Sarychew index to zero on each $[t_0',t_1']$. Now each of these subintervals can be further divided by Lem.~\ref{lem:existence_min_2_jets} to guarantee the existence of a finite minimal 2-jet for every possible $\wt b_1$. Now we apply Thm.~\ref{thm:optimal_deg_2} to each of the subintervals. 

{\new wypada³oby jeszcze wyt³umaczyæ siê z tego, ¿e w pierwszym kroku podzia³u bierzemy $[t_0',t_1']\subset(\tau_i,\tau_{i+1})$, a nie po prostu $[\tau_i,\tau_{i+1}]$. Niemniej poniewa¿ na ka¿dym $[t_0',t_1']$ mamy podzia³ na skoñczon¹ z góry ograniczon¹ liczbê czêci, to mo¿emy przejæ do maksymalnych podprzedzia³ów na których teza Tw.~\ref{thm:optimal_deg_2} zachodzi, wyczerpuj¹c ca³e $(\tau_i,\tau_{i+1})$.}
\end{proof}
